FastComposer: Tuning-Free Multi-Subject Image Generation with Localized Attention

Diffusion models excel at text-to-image generation, especially in subject-driven generation for personalized images. However, existing methods are inefficient due to the subject-specific fine-tuning, which is computationally intensive and hampers efficient deployment. Moreover, existing methods struggle with multi-subject generation as they often blend features among subjects. We present FastComposer which enables efficient, personalized, multi-subject text-to-image generation without fine-tuning. FastComposer uses subject embeddings extracted by an image encoder to augment the generic text conditioning in diffusion models, enabling personalized image generation based on subject images and textual instructions with only forward passes. To address the identity blending problem in the multi-subject generation, FastComposer proposes cross-attention localization supervision during training, enforcing the attention of reference subjects localized to the correct regions in the target images. Naively conditioning on subject embeddings results in subject overfitting. FastComposer proposes delayed subject conditioning in the denoising step to maintain both identity and editability in subject-driven image generation. FastComposer generates images of multiple unseen individuals with different styles, actions, and contexts. It achieves 300$\times$-2500$\times$ speedup compared to fine-tuning-based methods and requires zero extra storage for new subjects. FastComposer paves the way for efficient, personalized, and high-quality multi-subject image creation. Code, model, and dataset are available at https://github.com/mit-han-lab/fastcomposer.

==> figtab/fig_1.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/figure1.pdf}
    \caption{}
    \label{fig:1}
\end{figure*}

==> figtab/fig_inference.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
    \small
    \centering
    \includegraphics[width=0.6\textwidth]{figure/inference.pdf}
    \caption{Inference pipeline of \method.}
    \label{fig:inference}
\end{wrapfigure}

==> figtab/fig_subject3.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.5\linewidth]{figure/subjects3.pdf}
    \caption{Generating images with three subjects.}
    \label{fig:subject3}
\end{figure*}

==> figtab/fig_training.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure/training.pdf}
    \caption{Training pipeline of \method. Given a text description and images of multiple subjects, \method uses an image encoder to extract the features of the subjects, and augments the corresponding text tokens with the features. Then, the diffusion model is trained to generate multi-subject images.\fredo{make training/test clear.}}
    \label{fig:training}
\end{figure*}

==> figtab/tab_attn_loc.tex <==
\begin{wraptable}{r}{0.45\linewidth}
\setlength{\tabcolsep}{3.0pt}
    \centering
    \small
    \caption{Ablation studies on the cross-attention localization supervision. We compare with the model trained in the same setting without cross-attention localization.}
    \label{tab:abalation_loc}

    \begin{tabular}{lccc}
        \toprule
        Method         & Identity Pres. $\uparrow$ & Prompt Cons. $\uparrow$ & \\
        \midrule
        w/o Loc.       & 37.66\%              & \textbf{25.03\%}             \\
        w/ Loc. (Ours) & \textbf{43.11\%}      & 24.25\%      \\
        \bottomrule
    \end{tabular}
\end{wraptable}

==> figtab/tab_mixing_ablation.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Ablation studies on the ratio of subject-conditioning $\alpha$. TODO: Change this into a figure}
    \label{tab:mixing_ablation}

    \begin{tabular}{ccccc}
        \toprule
        Subject Conditioning Ratio & Identity Preservation $\uparrow$ & Prompt Consistency $\uparrow$ & \\
        \midrule
         1.0 & 0.5945 & 0.1854\\ 
         0.8 & 0.5745 & 0.2140 \\ 
         0.6 & 0.5156 & 0.2258\\ 
         0.5 & 0.4785 & 0.2346\\
         0.4 & 0.4279 & 0.2423\\
         0.2 & 0.2875 & 0.2502\\
         0.0 & 0.0716 & 0.2559\\ 
        \bottomrule
    \end{tabular}
\end{table}

==> text/7_conclusion.tex <==
\section{Conclusion}
We propose \method, a tuning-free method for personalized, multi-subject text-to-image generation. We achieve tuning-free subject-driven image generation by utilizing a pre-trained vision encoder, making this process efficient and accessible across various platforms. We also propose a novel delayed subject conditioning technique to balance the preservation of subject identity and the flexibility of image editability. Additionally, \method effectively tackles the identity blending issue in multi-subject generation by supervising cross-attention maps during pre-training. \method enables the creation of high-quality, personalized, and complex images, opening up new possibilities in the field of text-to-image generation.
